Cloud Resource Optimization for Processing Multiple Streams of Visual Data

Hundreds of millions of network cameras have been installed throughout the world. Each is capable of providing a vast amount of real-time data. Analyzing the massive data generated by these cameras requires significant computational resources and the demands may vary over time. Cloud computing shows the most promise to provide the needed resources on demand. In this article, we investigate how to allocate cloud resources when analyzing real-time data streams from network cameras. A resource manager considers many factors that affect its decisions, including the types of analysis, the number of data streams, and the locations of the cameras. The manager then selects the most cost-efficient types of cloud instances (e.g. CPU vs. GPGPU) to meet the computational demands for analyzing streams. We evaluate the effectiveness of our approach using Amazon Web Services. Experiments demonstrate more than 50% cost reduction for real workloads.

==> cover_letter.tex <==
Dear Editors and Reviewers: \newline
This paper is invited by Dr. El Saddik. Please see the e-mail below.

Thank You.\newline 

\begin{tt}
On 05/11/2018 11:53 PM, Abdulmotaleb El Saddik wrote:\newline

Dear Colleagues,
 
I hope this email finds you well. I am writing you today to congratulate you about your excellent work and to inform you that your paper titled “ANALYZING REAL-TIME MULTIMEDIA CONTENT FROM NETWORK CAMERAS USING CPUS AND GPUS IN THE CLOUD” was among the top 8 papers at IEEE MIPR 2018.  Hence it is my pleasure to invite you to submit an extended version of your paper to to a special issue of IEEE MultiMedia Magazine \newline
(https://publications.computer.org/multimedia-magazine/)\newline
 
Please submit the extended version of your paper by July 31, 2018 using our submission web site (https://mc.manuscriptcentral.com/cs-ieee)
Please do not hesitate to contact me if you need any further information or if you have any question. I will be happy to answer.\newline 
 
Best regards
-- Abed
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
Dr.-Ing.  Abdulmotaleb El Saddik     FIEEE, FCAE, FEIC, P.Eng.
Distinguished University Professor and University Research Chair

Director: Medical Devices Innovation Institute (MDII)

Director: Multimedia Communications Research Laboratory (MCRLab)

School of Electrical Engineering and Computer Science (EECS)

University of Ottawa

Email: elsaddik@uottawa.ca  | Web:   http://www.site.uottawa.ca/elsaddik
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
L’Université canadienne / Canada’s University

\end{tt}

==> future_cloud_computing.tex <==
% \vspace{-0.15cm}
% \section*{Cloud Resource Optimization for Processing Billions of Data Streams}\label{sec:cloud_future} 
% \vspace{-0.05cm}

Digital cameras have become fairly inexpensive and they can be deployed in many systems, called ``Internet of Video Things''~\cite{6410856}. It is expected that billions of cameras will be connected to the Internet capturing visual data continuously~\cite{8050296}. As computer vision technologies become mature, it is expected that most of the data streams will be analyzed in real-time. Analyzing the vast amounts of data would impose significant challenges.  The problem of optimizing cloud resources for processing billions of data streams would become an increasingly important problem.  The study presented in the paper is expected to be the beginning of a new research direction.


\begin{comment}



According to a report \cite{ihs_2017} in 2017, the global market for video surveillance will maintain an annual growth rate of less than 7\%. IHS also reported there were 49 million professionally operated and active global network cameras in 2014 \cite{ihs_2014} with sales of 66 million \cite{ihs_2016}, and 98 million \cite{ihs_2017} network cameras worldwide for the years 2016, and 2017, respectively. Since IHS did not report the number of sales in 2015, we will fit the trend and assume 30 million were shipped. This would sum to approximately 243 million total global network cameras currently in professional operation. As a conservative estimate we are going to assume a growth of an additional 5\% of network cameras being added to the global network per year. This compounded growth would result in approximately 450 million network cameras in operation worldwide by the year 2030.

We use {'}s approximation that the average network camera by 2030 would have an average resolution of 10MP. Now we are going to imagine a situation where every owner of each of these 450 million network cameras in 2030 wanted to download all the video data from these cameras at 30 frames per second and perform video analysis for a consecutive 24-hour period. This would result in more than 75 PB of data and roughly 2.5 million images from each camera. This is a huge amount of information that would need to be analyzed. If we are looking to estimate the amount of time and money it will cost to process all this information, then we must also take into consideration the rate at which GPU performance is growing. \cite{gpu_speed} claims GPU performance is growing, on average, at a rate of approximately 50\% year-over-year while data is growing at about 40\% year-over-year. If we assume a 10\% price decrease in GPU cloud usage year-over-year and an Amazon EC2 g2.2xlarge instance costs \$0.650 per hour in 2018, then by the year 2030 it would cost about \$0.184 per hour to use. YOLO, a popular object detection neural architecture, runs at 55 frames per second in 2018 on a Pascal Titan X GPU. If we continue to use the assumption that GPU’s will perform 50\% better year over year, YOLO will be able to process approximately 7,000 frames per second by the year 2030. If we wanted a single GPU to perform person tracking on all the images (2.5 million per day) from all the network cameras in the world in 2030 (450 million) then it would take that single GPU 18 million days to process, assuming a Pascal Titan X and an Amazon EC2 g2.2xlarge instance have similar processing speeds. At the price of \$0.184 per hour, it would cost 82 million dollars to process 24 hours of video and approximately 30 billion dollars for a years’ worth of video.

Although this situation is highly speculative, the need for a more cost and time efficient way of analyzing video data in the cloud, such as CPU and GPU optimization, still holds. [8] showed that their cloud resource manager can reduce cost by up to 61\% of the original price. If we assumed a 50\% price reduction by using a cloud resource manager, we could be saving nearly 15 billion dollars a year by 2030 on cloud video analytics. 



According to a report [1] in 2017, the global market for video surveillance will maintain an annual growth rate of less than 7\%. IHS also reported there were 49 million professionally operated and active global network cameras in 2014 with sales of “FILL THIS IN”, 66 million, and 98 million network cameras worldwide for the years 2015, 2016, and 2017, respectively. This would sum to “FILL THIS IN” total global network cameras currently in professional operation. As a conservative estimate we are going to assume growth of an additional 5\% of network cameras being added to the global network per year. This compounded growth would result in approximately 450 million network cameras in operation worldwide by the year 2030.


We use [5]’s approximation that the average network camera to 2030 would have an average resolution of 10MP and would stream data at approximately 30 frames per second. This would amount to one camera streaming more than 1 PB of data per day. Now we are going to imagine a situation where every owner of each of these 450 million network cameras in 2030 wanted to download all the video data from these cameras and perform video analysis for consecutive 24-hour period. This would result in more than 1e22 bytes of data and roughly 1e15 images. This is a significant amount of information that would need to be processed, stored, and analyzed. If we used YOLO, an object detection neural network architecture, running at approximately 55 frames per second to perform person tracking on all these images it would take approximately 2e9 hours to process. This of course would be impossible for any single computer to process and emphasizes the need for distributed cloud computing. According to [7], an Amazon EC2 g2.2xlarge instance costs \$0.650 per hour to use. At this price it would cost 1.3 billion dollars to process all the images from all the network cameras in the world in 2030 or about 470 billion dollars for the entire years’ worth of network camera data.
This shows an obvious need for a more cost-efficient way of analyzing video data in the cloud, such as CPU and GPU optimization. [8] showed that their cloud resource manager can reduce cost up to 61\% of the original price. If we assumed a 50\% price reduction by using a cloud resource manager, we could be saving nearly 250 billion dollars a year by 2030 and that is only within the field video analytics. 
\end{comment}

\begin{comment}
	Cloud computing has dramatically shaped the landscape of the digital world, yet we seem to only be at the start of the cloud era. In 2017, \$20 billion was spent on real estate for data centers in North America which totals more than the three previous years combined \cite{cbrae}. Cloud computing is already being taken advantage of across the spectrum from applications such as Facebook and Google Apps to services like Microsoft Azure and Amazon Web Services, however we seen to be at the beginning of the cloud era. A predicted 83\% of enterprises are expected to be offloading their workloads in the cloud by 2020 with approximately 41\% being on public cloud platforms, 20\% on private cloud platform and another 22\% on hybrid cloud platforms \cite{enterprisework}. We should expect to see exciting new innovations in the coming years as well as continued heightened investment into the cloud industry.

	Since cloud computing is relatively new, we will see in the upcoming years many new products and services being offered to further serve businesses and individual users alike. A service we can expect to see on the rise in upcoming years is Mobile Cloud Computing (MCC). Mobile devices have become an integral part of many of our lives and as mobile applications demand more computing resources and people demand lighter more portable devices there must be a shift of where this computing is being done, that is the cloud. According to \cite{mcc}, the global mobile cloud market is predicted to have a market value of \$66 billionn. The projected key players in MCC are AWS, Oracle, Inc., Microsoft, Google, and IBM. The  Potential applications for MCC could be cloud storage, cloud mobile media, learning and education, mobile social networks, mobile gaming, and cloud assisted Internet of Things (IOT). Some of the problems that MCC faces will gradually be handled over time. One of such problems that exists is access management to cloud servers. However, this can be handled by taking advantage of location information and by using context from mobile devices, so the cloud service providers can efficiently manage cloud resources to mobile users \cite{al2017mobile}. Understanding location data can help lead to more efficient offloading of computations by sending requests to cloud servers that are closer to the user, eliminating excessive transmission times. However, offloading all this data to the cloud may lead to frustration among users if the cloud service providers are not being clear about their intentions or usage. We have already seen the European Union acting by passing the General Data Protection Regulation or GDPR which demands for more transparent behavior from tech companies who utilize personal data. As cloud service providers continue to compete to become leaders of the cloud industry, we should expect to see immature companies who lack public trust and flexible platforms to drop out of the market while the most competitive will continue to thrive, offering cheaper prices, essential security measures, and greener technology (better management of resources such as cpu/gpu optimization and better allocation of cloud instances) \cite{penzel2015future}.
   
    At CAM$^2$ we are seeking to make advances in our optimizer to address these upcoming cloud computing concerns. For example, as cloud computing is growing all around the world, we want to make all types of data available to users. In the past, to keep our tests simple we chose to use only MJPEG data at specific frame rate and size; we are now planning to include other formats such as H.264 video data, and networks with a range of target frame rates and sizes in each of the cameras. Also, since our location based optimizer is exclusively testing on Amazon EC2 M3 instances, in the future we would like to implement a method to combine the benefits of both of our current resource managers. This new manager can then take into account not only the location of an instance, but also the range of available instances at that location. In the case of Amazon EC2, we would take into consideration M4, M5, G2, G3, and many more instance types while also optimizing for physical locations of those instances. . 

It is important to note however, that even today, we are making huge strides. In our best cases, we saw potential cost savings of over 60\%. This already can drastically impact savings in the cloud. In a 2018 study of 997 technical professionals, Right Scale found that 26\% of enterprises spend more than \$ 6 million a year on public cloud. If even just one of these companies was inefficiently using the cloud, our research shows they could potentially be overspending by over \$ 3,600,000. Because of this potentially significant wasted cloud spend, 58 \% of companies reported that optimizing cloud cost is among the top initiatives – a 5 \% increase from 2017. Therefore, as we grow our optimizer, even optimizing with the techniques we have today is critical when analyzing large-scale multimedia data.

\end{comment}

==> response.tex <==
\onecolumn
\section*{Response to Reviewers}

The authors want to thank
the editor and the reviewers
for their questions and suggestions.

\vspace{0.2in}

\noindent\begin{tabular}{|p{6in}|} \hline
{\tt The reviewers' comments are enclosed in this format.} \\ \hline
\end{tabular}
\subsection{Reviewer 1}
\vspace{0.2in}
\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
Comments: \newline
This manuscript introduces a resource management system to minimize the cost of cloud instances for globally distributed camera stream processing. The detailed comments are as follows. \newline
(1)     It can be confusing to the readers that the technique to consider both types and locations is mentioned in the “local optimization of cloud instances” section. The organization should be improved to illustrate the relationships among the proposed system, the instance type selection, and the local optimization.
}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} Thank you for your suggestions. We clarified the confusion by adding subsections into the paper. We separated the "CPU and GPU Management In The Cloud" section on Page \pageref{sec:cpu_gpu_optim} into 2 subsections: 1) "Differences Between CPUs and GPUs" and 2) "Select Instances with CPU and GPU". We also separated the "Local Optimization Of Cloud Instances" section on Page \pageref{location_section} (now renamed "Optimizing Instance Type And Location") into 2 subsections: 1) "Local Optimization", and 2) "Instance Type Optimization". We also rephrased the end of the  "CPU and GPU Management In The Cloud" section to clarify the relationship between these two main sections of the paper, and how the second part of the paper builds on the first. 

\vspace{0.2in}

\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
(2)     How to solve the multi-dimensional multi-choice packing problem is not explained clearly. This problem is important to the resource management system and more details of its solution should be provided.\newline
}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} We added a third paragraph and a figure in the Mult-Dimensional Multi-Choice Packing Problem side bar on Page \pageref{packing_problem_sidebar}. In this paragraph we explain our method of the multiple choice vector bin packing algorithm, and how it can be solved using a graph. The mathematics behind the graph compressor and the Gurobi solver are beyond the scope of this article, but we cite the sources that include more information on these topics.

\begin{comment}This is addressed with an additional paragraph in the Mult-Dimensional Multi-Choice Packing Problem side bar on Page \pageref{packing_problem_sidebar}. The paragraph explains how to formulate the problem so that it may be solved by a variety of different graph solving algorithms. The implementations of these solvers are often provided by specific platforms like Gurobi - the platform used by Brandao et al. It is beyond the scope of this article to go into great detail with regards to their implementation. {\bf Zohar: do you mean implementations or mathematics?}
\end{comment}
\vspace{0.2in}

\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
(3)     This manuscript involves system implementation and integration of the algorithms proposed in the authors’ previous papers. It will be better if the authors provide some justifications of its contribution with respect to system implementation and integration.\newline
}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} We added justification by providing more information on our evaluation and results. This information can be found in the "Optimizing Instance Location and Type" section on Page \pageref{sec:GCL_reference} and "CPU and GPU Management In The Cloud" section on Page \pageref{results_CPU}. These sections include our solution and our evaluation results. 
The contributions of this paper include (1) explanation of different resource management solutions
in different scenarios, (2) comparison of these algorithms in the context of large amounts 
of streaming data from network cameras, and (3) implementation of these methods on
commercial cloud (Amazon EC2).

% As for the justification of why we used a particular algorithm or method, such as the multiple choice vector bin packing method, we believe these justifications are out of scope for this magazine article. This information, however, can be found in the papers we cited.

\vspace{0.2in}

\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
(4)     The proposed system aims to minimize the cost without sacrificing performance. However, the authors need to provide enough results/data to show (a) whether the performance reduces when the cost decreases and (b) how the performance changes in each sample case.\newline
}
\\ 
\hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} In regard to CPU/GPU optimization, the system is designed to maintain at least 90\% performance. This is addressed in paragraph 4 of CPU and GPU Management in the Cloud section on Page \pageref{sec:cpu_gpu_optim}. This system is not intended to maximize performance with respect to cost, it is intended to maintain a minimum level of performance while minimizing cost with respect to CPU/GPU selection. We have added a table (figure \ref{fig:costSavings_CPUGPU}) in the CPU and GPU Management in the Cloud section that evaluates the cost of multiple instance selection strategies under three different scenarios. In regard to the Optimizing Instance Type and Location section, we have added another graphic (Figure \ref{fig:costComparison_frameRates}) to show how the cost of three different resource managers respond to different target frame rates. We also added citations to papers for a more detailed evaluation.


\vspace{0.2in}
\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
Additional Questions: \newline
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Very Relevant \newline
1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: This manuscript introduces a resource management system to minimize the cost of cloud instances (e.g., Amazon EC2 and Microsoft Azure) without sacrificing performance for the globally distributed network camera system, CAM$^2$. To deliver this challenge, two levels of optimizations were conducted to consider the instance’s type and its location simultaneously. First, a proper location is selected, based on the distance between the camera and the instance and the workload of the instance. Second, a proper instance’s type is selected with respect to the CPU, memory size, GPU, and GPU memory size. \newline
2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: Appears to be - but didn't check completely\newline
3. What do you see as this manuscript's contribution to the literature in this field? If you don't have any comments, please type No Comments.: No Comments\newline
4. What do you see as the strongest aspect of this manuscript? If you don't have any comments, please type No Comments.: No Comments\newline
5. What do you see as the weakest aspect of this manuscript? If you don't have any comments, please type No Comments.: No Comments\newline
1. If the title, abstract, and/or keywords are satisfactory, please denote this by placing a checkmark beside each one. Please elaborate in the Detailed Comments section.: Keywords. Abstract. Title\newline
2. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: References are sufficient and appropriate\newline
3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? please explain your answer in the Detailed Comments section.: Yes\newline
}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} Thank you for your feedback, we appreciate your comments.

\vspace{0.2in}
\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
4. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Could be improved\newline
}
\\ \hline
\end{tabular}

\vspace{0.2in}

{\bf Response:} Thank you for your feedback.  We have reorganized the paper.


\vspace{0.2in}

\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
5. Is the manuscript focused? Please elaborate in the Detailed Comments section.: Yes\newline
6. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Yes\newline
7. Please rate the readability of this manuscript in the Detailed Comments section.: Easy to read\newline
}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} Thank you for your feedback, we appreciate your comments. 


\subsection{Reviewer 2}

\vspace{0.2in}
\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
Comments:\newline
Two minor issues that should be revised in the manuscript.\newline
\newline Page 3, Table I: \newline
It would be good to indicate that the prices are in US\$. Maybe this could be
added in the top row: "Price Per Hour (US\$)". The MultiMedia magazine may be
read in different parts of the world and hence such a clarification would be
helpful.\newline
\newline Page 9, Acknowledgements: \newline
"We thank the the" -> remove second 'the'\newline
}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} We clarified that prices in Table \ref{table:cloudprice} are in US\$ and removed the second "the" in our Acknowledgements section on Page \pageref{sec:acknowledgements}.

\vspace{0.2in}
\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
Additional Questions:\newline
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Very Relevant

1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: The authors describe the fundamental and complex optimization problem that
arises if many camera streams need to be analyzed in a system environment that
utilizes world-wide distributed cloud computing resources. The different
factors that affect the computations and ultimately the overall system price
are described in an easily accessible fashion. Since the number of deployed
cameras is constantly increasing I believe this is an interesting topic.

2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: Yes

3. What do you see as this manuscript's contribution to the literature in this field? If you don't have any comments, please type No Comments.: The paper explains a complex, world-wide optimization problem in the context
of processing a multitude of video streams. I belief this is an area of
research which will increase in importance in the future.

4. What do you see as the strongest aspect of this manuscript? If you don't have any comments, please type No Comments.: Overall I think this paper describes the multi-dimensional multi-choice
packing problem that arises in a world-wide distributed camera stream
processing system in a way that is very accessible for most readers.


}
\\ \hline
\end{tabular}
\vspace{0.2in}

{\bf Response:} Thank you for your feedback, we appreciate your comments.
\vspace{0.2in}


\noindent\begin{tabular}{|p{6in}|} \hline
{\tt
5. What do you see as the weakest aspect of this manuscript? If you don't have any comments, please type No Comments.: One aspect that was not mentioned was that some resources or requirements might be changeable almost on a continuous scale, rather than at only discrete
steps. For example, the acceptable fps might be within a certain range. I
understand that not too many details can be explained in this article, but
maybe this issue could be mentioned in a sentence or two.
}
\\ \hline
\end{tabular}

\vspace{0.2in}

{\bf Response:} We added to the end of the "Optimizing Instance Type And Location" on Page \pageref{sec:GCL_reference} to address constantly changing resource requirements.
\vspace{0.2in}

\noindent\begin{tabular}{|p{6in}|} \hline
{\tt

1. If the title, abstract, and/or keywords are satisfactory, please denote this by placing a checkmark beside each one. Please elaborate in the Detailed Comments section.: Keywords. Abstract. Title

2. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: References are sufficient and appropriate

3. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? please explain your answer in the Detailed Comments section.: Yes

4. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Satisfactory

5. Is the manuscript focused? Please elaborate in the Detailed Comments section.: Yes

6. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Yes

7. Please rate the readability of this manuscript in the Detailed Comments section.: Easy to read
}
\\ \hline
\end{tabular} 

\vspace{0.2in}
{\bf Response:} Thank you for your feedback, we appreciate your comments.


